Empirically Evaluating the Use of Bytecode for Diversity-Based Test Case Prioritisation

Regression testing assures software correctness after changes but is resource-intensive. Test Case Prioritisation (TCP) mitigates this by ordering tests to maximise early fault detection. Diversity-based TCP prioritises dissimilar tests, assuming they exercise different system parts and uncover more faults. Traditional static diversity-based TCP approaches (i.e., methods that utilise the dissimilarity of tests), like the state-of-the-art FAST approach, rely on textual diversity from test source code, which is effective but inefficient due to its relative verbosity and redundancies affecting similarity calculations. This paper is the first to study bytecode as the basis of diversity in TCP, leveraging its compactness for improved efficiency and accuracy. An empirical study on seven Defects4J projects shows that bytecode diversity improves fault detection by 2.3-7.8% over text-based TCP. It is also 2-3 orders of magnitude faster in one TCP approach and 2.5-6 times faster in FAST-based TCP. Filtering specific bytecode instructions improves efficiency up to fourfold while maintaining effectiveness, making bytecode diversity a superior static approach.

==> figures/RQ1.tex <==
\begin{figure*}[htbp]
    \centering
    % Subfigure a
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphics/RQ1-APFD.pdf} 
        \vspace{-2em}
        \caption{APFD}
        \label{fig:RQ1-1}
    \end{subfigure}
    % Subfigure b
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphics/RQ1-RF.pdf} 
        \vspace{-2em}
        \caption{Real-fault detection}
        \label{fig:RQ1-2}
    \end{subfigure}
    \vspace{-1em}
    % Caption for the entire figure
    \caption{APFD and real-fault detection for static diversity-based TCP approaches}
    \label{fig:RQ1}
    \vspace{-1em}
\end{figure*}

==> figures/RQ2.tex <==
\begin{figure*}[htbp]
    \centering
    % Subfigure a
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphics/RQ2-1NEW.pdf} 
        \caption{APFD}
        \label{fig:RQ2-1}
    \end{subfigure}
    % Subfigure b
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{graphics/RQ2-2NEW.pdf} 
        \caption{Real-fault detection}
        \label{fig:RQ2-2}
    \end{subfigure}
    
    % Caption for the entire figure
    \caption{APFD and real-fault detection for bytecode-diversity and coverage-based TCP approaches}
    \label{fig:RQ2}
\end{figure*}

==> sections/abstract.tex <==
\begin{abstract}


% Shorter version:
% Regression testing assures software correctness after changes but is resource-intensive.
% %
% Test Case Prioritisation (TCP) optimises testing by ordering test cases to maximise early fault detection if testing needs to stop prematurely.
% %
% Diversity-based TCP is a key approach that prioritises test cases based on their dissimilarity, under the rationale that diverse tests are more likely to exercise different parts of the system and uncover more faults.
% %
% Traditional static diversity-based TCP approaches (\ie, methods that utilise the dissimilarity of tests), like the state-of-the-art FAST approach, use textual diversity based on test case source code, which is effective but inefficient due to its relative verbosity and redundancies such as whitespace, affecting similarity calculations.
% %
% This paper is the first to study bytecode as the basis of diversity in TCP. It leverages the compact, intermediate code of test cases to improve efficiency and accuracy.
% %
% An empirical evaluation using seven Defects4J projects shows that bytecode diversity achieves a~2.3–7.8\% higher fault detection rate than text-based TCP.
% %
% It is also 2–3 orders of magnitude faster in one TCP approach and 2.5–6 times faster when used in FAST-based TCP.
% %
% Filtering specific bytecode instructions improves efficiency up to fourfold while maintaining effectiveness, making bytecode diversity a superior static approach.

% Even shorter version:
Regression testing assures software correctness after changes but is resource-intensive. 
%
Test Case Prioritisation (TCP) mitigates this by ordering tests to maximise early fault detection. 
%
Diversity-based TCP prioritises dissimilar tests, assuming they exercise different system parts and uncover more faults. 
%
Traditional static diversity-based TCP approaches (\ie, methods that utilise the dissimilarity of tests), like the state-of-the-art FAST approach, rely on textual diversity from test source code, which is effective but inefficient due to its relative verbosity and redundancies affecting similarity calculations. 
%
This paper is the first to study bytecode as the basis of diversity in TCP, leveraging its compactness for improved efficiency and accuracy. 
%
An empirical study on seven Defects4J projects shows that bytecode diversity improves fault detection by 2.3–7.8\% over text-based TCP. 
%
It is also 2–3 orders of magnitude faster in one TCP approach and 2.5–6 times faster in FAST-based TCP. 
%
Filtering specific bytecode instructions improves efficiency up to fourfold while maintaining effectiveness, making bytecode diversity a superior static approach. 


\end{abstract}

